TransPimLib: A Library for Efficient Transcendental Functions on Processing-in-Memory Systems

Processing-in-memory (PIM) promises to alleviate the data movement bottleneck in modern computing systems. However, current real-world PIM systems have the inherent disadvantage that their hardware is more constrained than in conventional processors (CPU, GPU), due to the difficulty and cost of building processing elements near or inside the memory. As a result, general-purpose PIM architectures support fairly limited instruction sets and struggle to execute complex operations such as transcendental functions and other hard-to-calculate operations (e.g., square root). These operations are particularly important for some modern workloads, e.g., activation functions in machine learning applications. In order to provide support for transcendental (and other hard-to-calculate) functions in general-purpose PIM systems, we present \emph{TransPimLib}, a library that provides CORDIC-based and LUT-based methods for trigonometric functions, hyperbolic functions, exponentiation, logarithm, square root, etc. We develop an implementation of TransPimLib for the UPMEM PIM architecture and perform a thorough evaluation of TransPimLib's methods in terms of performance and accuracy, using microbenchmarks and three full workloads (Blackscholes, Sigmoid, Softmax). We open-source all our code and datasets at~\url{https://github.com/CMU-SAFARI/transpimlib}.

==> figures/tab-cordicoperations.tex <==
\begin{tabular}{p{36mm}p{16mm}p{16mm}llrrr}
\textbf{Modus}
& Matrix
& Variable \newline to Minimize 
& Input $v_0$   
& Input $\theta_0$  
& Output $v_n$ 
& Output $\theta_n$  \\ 
\hline

Circular Rotation
& Circular   
& $\theta_i$
& $\begin{bmatrix}  1\\ 0 \end{bmatrix}$
& $-x$ 
& $K_n  \cdot \begin{bmatrix} cos(x)\\ sin(x) \end{bmatrix} $  
& $0$  \\
\hline

Circular Vector
& Circular
& $v_0[1]$
& $\begin{bmatrix}  x\\ y \end{bmatrix}$
& $z$
& $K_n \begin{bmatrix} \sqrt{x^2 + y^2}\\ 0 \end{bmatrix}$
& $z + arctan(y / x)$ \\
\hline

Hyperbolic Rotation
& Hyperbolic 
& $\theta_i$
& $\begin{bmatrix}  1\\ 0 \end{bmatrix}  $
& $-x$
& $K_n \cdot \begin{bmatrix}  cosh(x)\\ sinh(x) \end{bmatrix} $ 
& $0$ \\
\hline

\multirow{5}{*}{Hyperbolic Vector}
& \multirow{5}{*}{Hyperbolic}
& \multirow{5}{*}{$v_0[1]$}
& $\begin{bmatrix}  x \\ y \end{bmatrix}$  
& $z$
& $K_n \cdot \begin{bmatrix}  \sqrt{x^2 - y^2} \\ 0 \end{bmatrix} $ 
& $z + Atanh(y/x)$  \\
\cline{3-7}

&
&
& $\begin{bmatrix}  x + 1 \\ x - 1 \end{bmatrix}$
& $0$
& $K_n \cdot \begin{bmatrix}  \sqrt{4x} \\ 0 \end{bmatrix} $ 
& $log(x) / 2$  \\
\cline{3-7}

&
&
& $\begin{bmatrix}  x + 0.25 \\ x - 0.25 \end{bmatrix} $ 
& $0$
& $K_n \cdot \begin{bmatrix}  \sqrt{x} \\ 0 \end{bmatrix} $ 
& $Atanh \left( \frac{x + 0.25}{x - 0.25}\right)$ \\
\hline

Linear Rotation
& Linear  
& $\theta_i$
& $\begin{bmatrix}  a \\ b \end{bmatrix}  $
& $c$
& $\begin{bmatrix} a \\ b + a \cdot c \end{bmatrix}  $
& $0$ \\
\hline

Linear Vector
& Linear  
& $v_0[1]$
& $\begin{bmatrix}  a \\ b \end{bmatrix}$ 
& $c$
& $\begin{bmatrix} a \\ 0  \end{bmatrix}  $
& $c + \frac{b}{a}$ \\
\end{tabular}

==> sections/05-discussion.tex <==
\section{Discussion}
\label{sec:discussion}

\todo{/*Discussion about generality of the library and its potential implementations on other real PIM architectures.*/}

\todo{Floating point not natively supported, fixed-point goes better despite multiplication.}

\todo{CORDIC methods may be better when instructions are natively supported.}

%There are works that use a similar methodology to our software solutions directly implemented in Hardware  specifically for machine learning activation functions \cite{skhynix_pim}. The key difference is the utilization of dedicated hardware for address generation and interpolation. The hardware based address generation does not seem to have any kind of configurable, which limits the types of address generation functions and their input ranges to the hardware specified values. This is most likely not an issue for the targeted machine learning applications, but might become an issue for more general purpose computing, but is most likely significantly faster than the software based approach. Address generation functions in our work are partially implemented using low manipulation of single bits, which would definitely be more efficient in dedicated hardware. Further research into configurable, high-performance address generation mechanisms and comparison of software and hardware solutions are needed to paint a full picture.
%This work largely specializes in an architecture where multiplication is expensive, and looks at options to calculate transcendental functions with minimal multiplicative effort. In other architectures \cite{samsung_pim}, multiplication might be readily available, which changes the landscape for transcendental function calls drastically. In architectures with fast multiplication, we expect functions without any usage of multiplications to perform similarly, while Lookup Table based methods (with typically one to two multiplications) speed up slightly, and multiplication heavy (such as Minimax Algorithms and Taylor Series) methods speed up significantly. Currently both the speed of multiplications in general, as well as implementations of transcendental functions are open research topics. 

